Falls Prediction in eldery people using Gated Recurrent Units

Falls prevention, especially in older people, becomes an increasingly important topic in the times of aging societies. In this work, we present Gated Recurrent Unit-based neural networks models designed for predicting falls (syncope). The cardiovascular systems signals used in the study come from Gravitational Physiology, Aging and Medicine Research Unit, Institute of Physiology, Medical University of Graz. We used two of the collected signals, heart rate, and mean blood pressure. By using bidirectional GRU model, it was possible to predict the syncope occurrence approximately ten minutes before the manual marker.

==> acronyms.tex <==
% CERN
\newacronym{LHC}{LHC}{Large Hadron Collider}
\newacronym{CERN}{CERN}{the European Organization for Nuclear Research}
\newacronym{PM}{PM}{Post Mortem}
\newacronym{PMS}{PM System}{\glsentrylong{PM} System}
\newacronym{PMF}{PM Framework}{\glsentrylong{PM} Framework}
\newacronym{LEP}{LEP}{Large Electron-Positron Collider}
\newacronym{PS}{PS}{Proton Synchrotron}
\newacronym{SPS}{SPS}{Super Proton Synchrotron}
\newacronym{ATLAS}{ATLAS}{A Toroidal LHC ApparatuS}
\newacronym{CMS}{CMS}{Compact Muon Solenoid}
\newacronym{ALICE}{ALICE}{A Large Ion Collider Experiment} \newacronym{LHCb}{LHCb}{Large Hadron Collider beauty experiment}
\newacronym{SUSY}{SUSY}{SUperSYmmetry}
\newacronym{SSB}{SSB}{Spontaneous Symmetry Breaking}
\newacronym{QPS}{QPS}{Quench Protection System}
\newacronym{SDDS}{SDDS}{Self-Describing Data Set}
\newacronym{MTF}{MTF}{Magnet Test Folder}
\newacronym{ELQA}{ELQA}{ELectrical Quality Assurance}

\newacronym{TE-MPE-EE}{TE-MPE-EE}{Technology Department --Machine Protection and Electrical Integrity group -- Electrical Engineering group}

% Deep Learning
\newacronym{DL}{DL}{Deep Learning}
\newacronym{LSTM}{LSTM}{Long Short-Term Memory}
\newacronym{GRU}{GRU}{Gated Recurrent Unit}
\newacronym{RMSE}{RMSE}{Root-Mean-Square Error}
\newacronym{RNN}{RNN}{Recurrent Neural Network}
\newacronym{ASIC}{ASIC}{Application-Specific Integrated Circuit}
\newacronym{FPGA}{FPGA}{Field-Programmable Gate Array}
\newacronym{FNN}{FNN}{Feed-forward Neural Network}
\newacronym{CNN}{CNN}{Convolutional Neural Network}

==> contents-10-materials-and-methods.tex <==
\section{Materials and methods}
\label{section:materials}


==> contents-30-discussion.tex <==
\section{Discussion}
\label{section:discussion}

==> quality_measures/accuracy.tex <==
\begin{equation}
    \mathrm{accuracy} = \frac{1}{N} \sum_{i=0}^{N-1} 1 \left( Y_i = \hat{Y}_i \right),
    \label{eq:class_accuracy}
\end{equation}

\noindent
where $Y_i$ and $\hat{Y}_i$ are the $i$-th sample true categories and ones predicted by the model, respectively, and $N$ is a dataset cardinality.


==> quality_measures/f_score_clusters.tex <==
An F-measure was used as a quality metric during conducted experiments. It is calculated using two helper metrics, a recall, also called sensitivity, and a precision. Given class $i$ and cluster $j$ those metrics are calculated as follows:

\begin{equation}
    \mathrm{recall}(i, j) = \frac{n_{ij}}{n_i},
    \label{eq:recall_clustering}
\end{equation}

\begin{equation}
    \mathrm{precision}(i, j) = \frac{n_{ij}}{n_j},
    \label{eq:precision_clustering}
\end{equation}

\noindent
where $n_{ij}$ is the number of items of class $i$ that are classified as members of cluster $j$, while $n_j$ and $n_i$ are the numbers of items in cluster $j$ and class $i$, respectively.

The clusters' $\mathrm{F}_\beta$ score is given by the following formula:

\begin{equation}
    \mathrm{F}_1(i, j) = (1 + \beta^2) \cdot \frac{\mathrm{recall}(i, j) \cdot \mathrm{precision}(i, j)}{\mathrm{recall}(i, j) + \beta^2 \cdot \mathrm{precision}(i, j)},
    \label{eq:fractional_F_measure}
\end{equation}

\noindent
where $\beta$ parameter controls the recall importance in relevance to the precision. For results presented in this paper $\beta=1$ was used.

The overall quality of the classification can be obtained by taking the weighted average $\mathrm{F}_1$ scores for each class. It is given by the equation:

\begin{equation}
    \mathrm{F}_1 = \sum\limits_{i} \frac{n_i}{n}\max{\mathrm{F}_1(i, j)},
    \label{eq:overall_F_measure}
\end{equation}

where the maximum is taken over all clusters and $n$ is the number of all objects. The $\mathrm{F}_1$ score value ranges from 0 to 1, with a higher value indicating a higher clustering quality.

==> quality_measures/rmse.tex <==
\begin{equation}
\mathrm{RMSE} = {\sqrt {\frac{1} {N}{\sum\limits_{i = 1}^N {\left({y}_{\mathit{r}}^{i} - y_{\mathit{p}}^{i} \right)^{2} }}}} 
  \label{eq:rmse}
\end{equation}

\begin{equation}
\mathrm{MPE} = {\frac{100 \%} {N}{\sum\limits_{i = 1}^N \frac{{{y}_{\mathit{r}}^{i} - y_{\mathit{p}}^{i}}}{{y}_{\mathit{r}}^{i}} } }
  \label{eq:mpe}
\end{equation}

\noindent
where: ${y}_{\mathit{r}}^{i}$ and $y_{\mathit{p}}^{i}$ are a voltage time series and its predicted counterpart, respectively, and $N$ is a dataset cardinality.
